Modular Meshed Ultra-Wideband Aided Inertial Navigation with Robust Anchor Calibration

This paper introduces a generic filter-based state estimation framework that supports two state-decoupling strategies based on cross-covariance factorization. These strategies reduce the computational complexity and inherently support true modularity -- a perquisite for handling and processing meshed range measurements among a time-varying set of devices. In order to utilize these measurements in the estimation framework, positions of newly detected stationary devices (anchors) and the pairwise biases between the ranging devices are required. In this work an autonomous calibration procedure for new anchors is presented, that utilizes range measurements from multiple tags as well as already known anchors. To improve the robustness, an outlier rejection method is introduced. After the calibration is performed, the sensor fusion framework obtains initial beliefs of the anchor positions and dictionaries of pairwise biases, in order to fuse range measurements obtained from new anchors tightly-coupled. The effectiveness of the filter and calibration framework has been validated through evaluations on a recorded dataset and real-world experiments.

==> styles/colors.tex <==
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\definecolor{Accent3qual1}{RGB}{127,201,127}
\definecolor{Accent3qual2}{RGB}{190,174,212}
\definecolor{Accent3qual3}{RGB}{253,192,134}
\definecolor{Accent5qual1}{RGB}{127,201,127}
\definecolor{Accent5qual2}{RGB}{190,174,212}
\definecolor{Accent5qual3}{RGB}{253,192,134}
\definecolor{Accent5qual4}{RGB}{255,255,153}
\definecolor{Accent5qual5}{RGB}{56,108,176}
\definecolor{Accent7qual1}{RGB}{127,201,127}
\definecolor{Accent7qual2}{RGB}{190,174,212}
\definecolor{Accent7qual3}{RGB}{253,192,134}
\definecolor{Accent7qual4}{RGB}{255,255,153}
\definecolor{Accent7qual5}{RGB}{56,108,176}
\definecolor{Accent7qual6}{RGB}{240,2,127}
\definecolor{Accent7qual7}{RGB}{191,91,23}

%EDIT: Added number of classes
\definecolor{Blues3seq1}{RGB}{222,235,247}
\definecolor{Blues3seq2}{RGB}{158,202,225}
\definecolor{Blues3seq3}{RGB}{49,130,189}

\definecolor{Blues4seq1}{RGB}{239,243,255}
\definecolor{Blues4seq2}{RGB}{189,215,231}
\definecolor{Blues4seq3}{RGB}{107,174,214}
\definecolor{Blues4seq4}{RGB}{33,113,181}

\definecolor{Blues5seq1}{RGB}{239,243,255}
\definecolor{Blues5seq2}{RGB}{189,215,231}
\definecolor{Blues5seq3}{RGB}{107,174,214}
\definecolor{Blues5seq4}{RGB}{49,130,189}
\definecolor{Blues5seq5}{RGB}{8,81,156}

\definecolor{Blues6seq1}{RGB}{239,243,255}
\definecolor{Blues6seq2}{RGB}{198,219,239}
\definecolor{Blues6seq3}{RGB}{158,202,225}
\definecolor{Blues6seq4}{RGB}{107,174,214}
\definecolor{Blues6seq5}{RGB}{49,130,189}
\definecolor{Blues6seq6}{RGB}{8,81,156}

\definecolor{Blues7seq1}{RGB}{239,243,255}
\definecolor{Blues7seq2}{RGB}{198,219,239}
\definecolor{Blues7seq3}{RGB}{158,202,225}
\definecolor{Blues7seq4}{RGB}{107,174,214}
\definecolor{Blues7seq5}{RGB}{66,146,198}
\definecolor{Blues7seq6}{RGB}{33,113,181}
\definecolor{Blues7seq7}{RGB}{8,69,148}

\definecolor{Blues8seq1}{RGB}{247,251,255}
\definecolor{Blues8seq2}{RGB}{222,235,247}
\definecolor{Blues8seq3}{RGB}{198,219,239}
\definecolor{Blues8seq4}{RGB}{158,202,225}
\definecolor{Blues8seq5}{RGB}{107,174,214}
\definecolor{Blues8seq6}{RGB}{66,146,198}
\definecolor{Blues8seq7}{RGB}{33,113,181}
\definecolor{Blues8seq8}{RGB}{8,69,148}

\definecolor{Blues9seq1}{RGB}{247,251,255}
\definecolor{Blues9seq2}{RGB}{222,235,247}
\definecolor{Blues9seq3}{RGB}{198,219,239}
\definecolor{Blues9seq4}{RGB}{158,202,225}
\definecolor{Blues9seq5}{RGB}{107,174,214}
\definecolor{Blues9seq6}{RGB}{66,146,198}
\definecolor{Blues9seq7}{RGB}{33,113,181}
\definecolor{Blues9seq8}{RGB}{8,81,156}
\definecolor{Blues9seq9}{RGB}{8,48,107}
%END EDIT

\definecolor{BrBG4div1}{RGB}{166,97,26}
\definecolor{BrBG4div2}{RGB}{223,194,125}
\definecolor{BrBG4div3}{RGB}{128,205,193}
\definecolor{BrBG4div4}{RGB}{1,133,113}
\definecolor{BrBG6div1}{RGB}{140,81,10}
\definecolor{BrBG6div2}{RGB}{216,179,101}
\definecolor{BrBG6div3}{RGB}{246,232,195}
\definecolor{BrBG6div4}{RGB}{199,234,229}
\definecolor{BrBG6div5}{RGB}{90,180,172}
\definecolor{BrBG6div6}{RGB}{1,102,94}
\definecolor{BrBG8div1}{RGB}{140,81,10}
\definecolor{BrBG8div2}{RGB}{191,129,45}
\definecolor{BrBG8div3}{RGB}{223,194,125}
\definecolor{BrBG8div4}{RGB}{246,232,195}
\definecolor{BrBG8div5}{RGB}{199,234,229}
\definecolor{BrBG8div6}{RGB}{128,205,193}
\definecolor{BrBG8div7}{RGB}{53,151,143}
\definecolor{BrBG8div8}{RGB}{1,102,94}
\definecolor{BrBG10div1}{RGB}{84,48,5}
\definecolor{BrBG10div2}{RGB}{140,81,10}
\definecolor{BrBG10div3}{RGB}{191,129,45}
\definecolor{BrBG10div4}{RGB}{223,194,125}
\definecolor{BrBG10div5}{RGB}{246,232,195}
\definecolor{BrBG10div6}{RGB}{199,234,229}
\definecolor{BrBG10div7}{RGB}{128,205,193}
\definecolor{BrBG10div8}{RGB}{53,151,143}
\definecolor{BrBG10div9}{RGB}{1,102,94}
\definecolor{BrBG10div10}{RGB}{0,60,48}
\definecolor{BuGn3seq1}{RGB}{229,245,249}
\definecolor{BuGn3seq2}{RGB}{153,216,201}
\definecolor{BuGn3seq3}{RGB}{44,162,95}
\definecolor{BuGn5seq1}{RGB}{237,248,251}
\definecolor{BuGn5seq2}{RGB}{178,226,226}
\definecolor{BuGn5seq3}{RGB}{102,194,164}
\definecolor{BuGn5seq4}{RGB}{44,162,95}
\definecolor{BuGn5seq5}{RGB}{0,109,44}
\definecolor{BuGn7seq1}{RGB}{237,248,251}
\definecolor{BuGn7seq2}{RGB}{204,236,230}
\definecolor{BuGn7seq3}{RGB}{153,216,201}
\definecolor{BuGn7seq4}{RGB}{102,194,164}
\definecolor{BuGn7seq5}{RGB}{65,174,118}
\definecolor{BuGn7seq6}{RGB}{35,139,69}
\definecolor{BuGn7seq7}{RGB}{0,88,36}
\definecolor{BuGn9seq1}{RGB}{247,252,253}
\definecolor{BuGn9seq2}{RGB}{229,245,249}
\definecolor{BuGn9seq3}{RGB}{204,236,230}
\definecolor{BuGn9seq4}{RGB}{153,216,201}
\definecolor{BuGn9seq5}{RGB}{102,194,164}
\definecolor{BuGn9seq6}{RGB}{65,174,118}
\definecolor{BuGn9seq7}{RGB}{35,139,69}
\definecolor{BuGn9seq8}{RGB}{0,109,44}
\definecolor{BuGn9seq9}{RGB}{0,68,27}
\definecolor{BuPu4seq1}{RGB}{237,248,251}
\definecolor{BuPu4seq2}{RGB}{179,205,227}
\definecolor{BuPu4seq3}{RGB}{140,150,198}
\definecolor{BuPu4seq4}{RGB}{136,65,157}
\definecolor{BuPu6seq1}{RGB}{237,248,251}
\definecolor{BuPu6seq2}{RGB}{191,211,230}
\definecolor{BuPu6seq3}{RGB}{158,188,218}
\definecolor{BuPu6seq4}{RGB}{140,150,198}
\definecolor{BuPu6seq5}{RGB}{136,86,167}
\definecolor{BuPu6seq6}{RGB}{129,15,124}
\definecolor{BuPu8seq1}{RGB}{247,252,253}
\definecolor{BuPu8seq2}{RGB}{224,236,244}
\definecolor{BuPu8seq3}{RGB}{191,211,230}
\definecolor{BuPu8seq4}{RGB}{158,188,218}
\definecolor{BuPu8seq5}{RGB}{140,150,198}
\definecolor{BuPu8seq6}{RGB}{140,107,177}
\definecolor{BuPu8seq7}{RGB}{136,65,157}
\definecolor{BuPu8seq8}{RGB}{110,1,107}
\definecolor{Dark23qual1}{RGB}{27,158,119}
\definecolor{Dark23qual2}{RGB}{217,95,2}
\definecolor{Dark23qual3}{RGB}{117,112,179}
\definecolor{Dark25qual1}{RGB}{27,158,119}
\definecolor{Dark25qual2}{RGB}{217,95,2}
\definecolor{Dark25qual3}{RGB}{117,112,179}
\definecolor{Dark25qual4}{RGB}{231,41,138}
\definecolor{Dark25qual5}{RGB}{102,166,30}
\definecolor{Dark27qual1}{RGB}{27,158,119}
\definecolor{Dark27qual2}{RGB}{217,95,2}
\definecolor{Dark27qual3}{RGB}{117,112,179}
\definecolor{Dark27qual4}{RGB}{231,41,138}
\definecolor{Dark27qual5}{RGB}{102,166,30}
\definecolor{Dark27qual6}{RGB}{230,171,2}
\definecolor{Dark27qual7}{RGB}{166,118,29}
\definecolor{GnBu3seq1}{RGB}{224,243,219}
\definecolor{GnBu3seq2}{RGB}{168,221,181}
\definecolor{GnBu3seq3}{RGB}{67,162,202}
\definecolor{GnBu5seq1}{RGB}{240,249,232}
\definecolor{GnBu5seq2}{RGB}{186,228,188}
\definecolor{GnBu5seq3}{RGB}{123,204,196}
\definecolor{GnBu5seq4}{RGB}{67,162,202}
\definecolor{GnBu5seq5}{RGB}{8,104,172}
\definecolor{GnBu7seq1}{RGB}{240,249,232}
\definecolor{GnBu7seq2}{RGB}{204,235,197}
\definecolor{GnBu7seq3}{RGB}{168,221,181}
\definecolor{GnBu7seq4}{RGB}{123,204,196}
\definecolor{GnBu7seq5}{RGB}{78,179,211}
\definecolor{GnBu7seq6}{RGB}{43,140,190}
\definecolor{GnBu7seq7}{RGB}{8,88,158}
\definecolor{GnBu9seq1}{RGB}{247,252,240}
\definecolor{GnBu9seq2}{RGB}{224,243,219}
\definecolor{GnBu9seq3}{RGB}{204,235,197}
\definecolor{GnBu9seq4}{RGB}{168,221,181}
\definecolor{GnBu9seq5}{RGB}{123,204,196}
\definecolor{GnBu9seq6}{RGB}{78,179,211}
\definecolor{GnBu9seq7}{RGB}{43,140,190}
\definecolor{GnBu9seq8}{RGB}{8,104,172}
\definecolor{GnBu9seq9}{RGB}{8,64,129}

%EDIT: Added number of classes 
\definecolor{Greens3seq1}{RGB}{237,248,233}
\definecolor{Greens3seq2}{RGB}{161,217,155}
\definecolor{Greens3seq3}{RGB}{49,163,84}

\definecolor{Greens4seq1}{RGB}{237,248,233}
\definecolor{Greens4seq2}{RGB}{186,228,179}
\definecolor{Greens4seq3}{RGB}{116,196,118}
\definecolor{Greens4seq4}{RGB}{35,139,69}

\definecolor{Greens5seq1}{RGB}{237,248,233}
\definecolor{Greens5seq2}{RGB}{186,228,179}
\definecolor{Greens5seq3}{RGB}{116,196,118}
\definecolor{Greens5seq4}{RGB}{49,163,84}
\definecolor{Greens5seq5}{RGB}{0,109,44}

\definecolor{Greens6seq1}{RGB}{237,248,233}
\definecolor{Greens6seq2}{RGB}{199,233,192}
\definecolor{Greens6seq3}{RGB}{161,217,155}
\definecolor{Greens6seq4}{RGB}{116,196,118}
\definecolor{Greens6seq5}{RGB}{49,163,84}
\definecolor{Greens6seq6}{RGB}{0,109,44}

\definecolor{Greens7seq1}{RGB}{237,248,233}
\definecolor{Greens7seq2}{RGB}{199,233,192}
\definecolor{Greens7seq3}{RGB}{161,217,155}
\definecolor{Greens7seq4}{RGB}{116,196,118}
\definecolor{Greens7seq5}{RGB}{65,171,93}
\definecolor{Greens7seq6}{RGB}{35,139,69}
\definecolor{Greens7seq7}{RGB}{0,90,50}

\definecolor{Greens8seq1}{RGB}{247,252,245}
\definecolor{Greens8seq2}{RGB}{229,245,224}
\definecolor{Greens8seq3}{RGB}{199,233,192}
\definecolor{Greens8seq4}{RGB}{161,217,155}
\definecolor{Greens8seq5}{RGB}{116,196,118}
\definecolor{Greens8seq6}{RGB}{65,171,93}
\definecolor{Greens8seq7}{RGB}{35,139,69}
\definecolor{Greens8seq8}{RGB}{0,90,50}

\definecolor{Greens9seq1}{RGB}{247,252,245}
\definecolor{Greens9seq2}{RGB}{229,245,224}
\definecolor{Greens9seq3}{RGB}{199,233,192}
\definecolor{Greens9seq4}{RGB}{161,217,155}
\definecolor{Greens9seq5}{RGB}{116,196,118}
\definecolor{Greens9seq6}{RGB}{65,171,93}
\definecolor{Greens9seq7}{RGB}{35,139,69}
\definecolor{Greens9seq8}{RGB}{0,109,44}
\definecolor{Greens9seq9}{RGB}{0,68,27}
%END EDIT

\definecolor{Greys3seq1}{RGB}{240,240,240}
\definecolor{Greys3seq2}{RGB}{189,189,189}
\definecolor{Greys3seq3}{RGB}{99,99,99}
\definecolor{Greys5seq1}{RGB}{247,247,247}
\definecolor{Greys5seq2}{RGB}{204,204,204}
\definecolor{Greys5seq3}{RGB}{150,150,150}
\definecolor{Greys5seq4}{RGB}{99,99,99}
\definecolor{Greys5seq5}{RGB}{37,37,37}
\definecolor{Greys7seq1}{RGB}{247,247,247}
\definecolor{Greys7seq2}{RGB}{217,217,217}
\definecolor{Greys7seq3}{RGB}{189,189,189}
\definecolor{Greys7seq4}{RGB}{150,150,150}
\definecolor{Greys7seq5}{RGB}{115,115,115}
\definecolor{Greys7seq6}{RGB}{82,82,82}
\definecolor{Greys7seq7}{RGB}{37,37,37}
\definecolor{Greys9seq1}{RGB}{255,255,255}
\definecolor{Greys9seq2}{RGB}{240,240,240}
\definecolor{Greys9seq3}{RGB}{217,217,217}
\definecolor{Greys9seq4}{RGB}{189,189,189}
\definecolor{Greys9seq5}{RGB}{150,150,150}
\definecolor{Greys9seq6}{RGB}{115,115,115}
\definecolor{Greys9seq7}{RGB}{82,82,82}
\definecolor{Greys9seq8}{RGB}{37,37,37}
\definecolor{Greys9seq9}{RGB}{0,0,0}
\definecolor{Oranges4seq1}{RGB}{254,237,222}
\definecolor{Oranges4seq2}{RGB}{253,190,133}
\definecolor{Oranges4seq3}{RGB}{253,141,60}
\definecolor{Oranges4seq4}{RGB}{217,71,1}
\definecolor{Oranges6seq1}{RGB}{254,237,222}
\definecolor{Oranges6seq2}{RGB}{253,208,162}
\definecolor{Oranges6seq3}{RGB}{253,174,107}
\definecolor{Oranges6seq4}{RGB}{253,141,60}
\definecolor{Oranges6seq5}{RGB}{230,85,13}
\definecolor{Oranges6seq6}{RGB}{166,54,3}
\definecolor{Oranges8seq1}{RGB}{255,245,235}
\definecolor{Oranges8seq2}{RGB}{254,230,206}
\definecolor{Oranges8seq3}{RGB}{253,208,162}
\definecolor{Oranges8seq4}{RGB}{253,174,107}
\definecolor{Oranges8seq5}{RGB}{253,141,60}
\definecolor{Oranges8seq6}{RGB}{241,105,19}
\definecolor{Oranges8seq7}{RGB}{217,72,1}
\definecolor{Oranges8seq8}{RGB}{140,45,4}
\definecolor{OrRd3seq1}{RGB}{254,232,200}
\definecolor{OrRd3seq2}{RGB}{253,187,132}
\definecolor{OrRd3seq3}{RGB}{227,74,51}
\definecolor{OrRd5seq1}{RGB}{254,240,217}
\definecolor{OrRd5seq2}{RGB}{253,204,138}
\definecolor{OrRd5seq3}{RGB}{252,141,89}
\definecolor{OrRd5seq4}{RGB}{227,74,51}
\definecolor{OrRd5seq5}{RGB}{179,0,0}
\definecolor{OrRd7seq1}{RGB}{254,240,217}
\definecolor{OrRd7seq2}{RGB}{253,212,158}
\definecolor{OrRd7seq3}{RGB}{253,187,132}
\definecolor{OrRd7seq4}{RGB}{252,141,89}
\definecolor{OrRd7seq5}{RGB}{239,101,72}
\definecolor{OrRd7seq6}{RGB}{215,48,31}
\definecolor{OrRd7seq7}{RGB}{153,0,0}
\definecolor{OrRd9seq1}{RGB}{255,247,236}
\definecolor{OrRd9seq2}{RGB}{254,232,200}
\definecolor{OrRd9seq3}{RGB}{253,212,158}
\definecolor{OrRd9seq4}{RGB}{253,187,132}
\definecolor{OrRd9seq5}{RGB}{252,141,89}
\definecolor{OrRd9seq6}{RGB}{239,101,72}
\definecolor{OrRd9seq7}{RGB}{215,48,31}
\definecolor{OrRd9seq8}{RGB}{179,0,0}
\definecolor{OrRd9seq9}{RGB}{127,0,0}

%EDIT: Added number of classes
\definecolor{Paired3qual1}{RGB}{166,206,227}
\definecolor{Paired3qual2}{RGB}{31,120,180}
\definecolor{Paired3qual3}{RGB}{178,223,138}

\definecolor{Paired4qual1}{RGB}{166,206,227}
\definecolor{Paired4qual2}{RGB}{31,120,180}
\definecolor{Paired4qual3}{RGB}{178,223,138}
\definecolor{Paired4qual4}{RGB}{51,160,44}

\definecolor{Paired5qual1}{RGB}{166,206,227}
\definecolor{Paired5qual2}{RGB}{31,120,180}
\definecolor{Paired5qual3}{RGB}{178,223,138}
\definecolor{Paired5qual4}{RGB}{51,160,44}
\definecolor{Paired5qual5}{RGB}{251,154,153}

\definecolor{Paired6qual1}{RGB}{166,206,227}
\definecolor{Paired6qual2}{RGB}{31,120,180}
\definecolor{Paired6qual3}{RGB}{178,223,138}
\definecolor{Paired6qual4}{RGB}{51,160,44}
\definecolor{Paired6qual5}{RGB}{251,154,153}
\definecolor{Paired6qual6}{RGB}{227,26,28}

\definecolor{Paired7qual1}{RGB}{166,206,227}
\definecolor{Paired7qual2}{RGB}{31,120,180}
\definecolor{Paired7qual3}{RGB}{178,223,138}
\definecolor{Paired7qual4}{RGB}{51,160,44}
\definecolor{Paired7qual5}{RGB}{251,154,153}
\definecolor{Paired7qual6}{RGB}{227,26,28}
\definecolor{Paired7qual7}{RGB}{253,191,111}

\definecolor{Paired8qual1}{RGB}{166,206,227}
\definecolor{Paired8qual2}{RGB}{31,120,180}
\definecolor{Paired8qual3}{RGB}{178,223,138}
\definecolor{Paired8qual4}{RGB}{51,160,44}
\definecolor{Paired8qual5}{RGB}{251,154,153}
\definecolor{Paired8qual6}{RGB}{227,26,28}
\definecolor{Paired8qual7}{RGB}{253,191,111}
\definecolor{Paired8qual8}{RGB}{255,127,0}

\definecolor{Paired9qual1}{RGB}{166,206,227}
\definecolor{Paired9qual2}{RGB}{31,120,180}
\definecolor{Paired9qual3}{RGB}{178,223,138}
\definecolor{Paired9qual4}{RGB}{51,160,44}
\definecolor{Paired9qual5}{RGB}{251,154,153}
\definecolor{Paired9qual6}{RGB}{227,26,28}
\definecolor{Paired9qual7}{RGB}{253,191,111}
\definecolor{Paired9qual8}{RGB}{255,127,0}
\definecolor{Paired9qual9}{RGB}{202,178,214}

\definecolor{Paired10qual1}{RGB}{166,206,227}
\definecolor{Paired10qual2}{RGB}{31,120,180}
\definecolor{Paired10qual3}{RGB}{178,223,138}
\definecolor{Paired10qual4}{RGB}{51,160,44}
\definecolor{Paired10qual5}{RGB}{251,154,153}
\definecolor{Paired10qual6}{RGB}{227,26,28}
\definecolor{Paired10qual7}{RGB}{253,191,111}
\definecolor{Paired10qual8}{RGB}{255,127,0}
\definecolor{Paired10qual9}{RGB}{202,178,214}
\definecolor{Paired10qual10}{RGB}{106,61,154}

\definecolor{Paired12qual1}{RGB}{166,206,227}
\definecolor{Paired12qual2}{RGB}{31,120,180}
\definecolor{Paired12qual3}{RGB}{178,223,138}
\definecolor{Paired12qual4}{RGB}{51,160,44}
\definecolor{Paired12qual5}{RGB}{251,154,153}
\definecolor{Paired12qual6}{RGB}{227,26,28}
\definecolor{Paired12qual7}{RGB}{253,191,111}
\definecolor{Paired12qual8}{RGB}{255,127,0}
\definecolor{Paired12qual9}{RGB}{202,178,214}
\definecolor{Paired12qual10}{RGB}{106,61,154}
\definecolor{Paired12qual11}{RGB}{255,255,153}
\definecolor{Paired12qual12}{RGB}{177,89,40}
%END EDIT

\definecolor{Pastel14qual1}{RGB}{251,180,174}
\definecolor{Pastel14qual2}{RGB}{179,205,227}
\definecolor{Pastel14qual3}{RGB}{204,235,197}
\definecolor{Pastel14qual4}{RGB}{222,203,228}
\definecolor{Pastel16qual1}{RGB}{251,180,174}
\definecolor{Pastel16qual2}{RGB}{179,205,227}
\definecolor{Pastel16qual3}{RGB}{204,235,197}
\definecolor{Pastel16qual4}{RGB}{222,203,228}
\definecolor{Pastel16qual5}{RGB}{254,217,166}
\definecolor{Pastel16qual6}{RGB}{255,255,204}
\definecolor{Pastel18qual1}{RGB}{251,180,174}
\definecolor{Pastel18qual2}{RGB}{179,205,227}
\definecolor{Pastel18qual3}{RGB}{204,235,197}
\definecolor{Pastel18qual4}{RGB}{222,203,228}
\definecolor{Pastel18qual5}{RGB}{254,217,166}
\definecolor{Pastel18qual6}{RGB}{255,255,204}
\definecolor{Pastel18qual7}{RGB}{229,216,189}
\definecolor{Pastel18qual8}{RGB}{253,218,236}
\definecolor{Pastel23qual1}{RGB}{179,226,205}
\definecolor{Pastel23qual2}{RGB}{253,205,172}
\definecolor{Pastel23qual3}{RGB}{203,213,232}
\definecolor{Pastel25qual1}{RGB}{179,226,205}
\definecolor{Pastel25qual2}{RGB}{253,205,172}
\definecolor{Pastel25qual3}{RGB}{203,213,232}
\definecolor{Pastel25qual4}{RGB}{244,202,228}
\definecolor{Pastel25qual5}{RGB}{230,245,201}
\definecolor{Pastel27qual1}{RGB}{179,226,205}
\definecolor{Pastel27qual2}{RGB}{253,205,172}
\definecolor{Pastel27qual3}{RGB}{203,213,232}
\definecolor{Pastel27qual4}{RGB}{244,202,228}
\definecolor{Pastel27qual5}{RGB}{230,245,201}
\definecolor{Pastel27qual6}{RGB}{255,242,174}
\definecolor{Pastel27qual7}{RGB}{241,226,204}
\definecolor{PiYG3div1}{RGB}{233,163,201}
\definecolor{PiYG3div2}{RGB}{247,247,247}
\definecolor{PiYG3div3}{RGB}{161,215,106}
\definecolor{PiYG5div1}{RGB}{208,28,139}
\definecolor{PiYG5div2}{RGB}{241,182,218}
\definecolor{PiYG5div3}{RGB}{247,247,247}
\definecolor{PiYG5div4}{RGB}{184,225,134}
\definecolor{PiYG5div5}{RGB}{77,172,38}
\definecolor{PiYG7div1}{RGB}{197,27,125}
\definecolor{PiYG7div2}{RGB}{233,163,201}
\definecolor{PiYG7div3}{RGB}{253,224,239}
\definecolor{PiYG7div4}{RGB}{247,247,247}
\definecolor{PiYG7div5}{RGB}{230,245,208}
\definecolor{PiYG7div6}{RGB}{161,215,106}
\definecolor{PiYG7div7}{RGB}{77,146,33}
\definecolor{PiYG9div1}{RGB}{197,27,125}
\definecolor{PiYG9div2}{RGB}{222,119,174}
\definecolor{PiYG9div3}{RGB}{241,182,218}
\definecolor{PiYG9div4}{RGB}{253,224,239}
\definecolor{PiYG9div5}{RGB}{247,247,247}
\definecolor{PiYG9div6}{RGB}{230,245,208}
\definecolor{PiYG9div7}{RGB}{184,225,134}
\definecolor{PiYG9div8}{RGB}{127,188,65}
\definecolor{PiYG9div9}{RGB}{77,146,33}
\definecolor{PiYG11div1}{RGB}{142,1,82}
\definecolor{PiYG11div2}{RGB}{197,27,125}
\definecolor{PiYG11div3}{RGB}{222,119,174}
\definecolor{PiYG11div4}{RGB}{241,182,218}
\definecolor{PiYG11div5}{RGB}{253,224,239}
\definecolor{PiYG11div6}{RGB}{247,247,247}
\definecolor{PiYG11div7}{RGB}{230,245,208}
\definecolor{PiYG11div8}{RGB}{184,225,134}
\definecolor{PiYG11div9}{RGB}{127,188,65}
\definecolor{PiYG11div10}{RGB}{77,146,33}
\definecolor{PiYG11div11}{RGB}{39,100,25}
\definecolor{PRGn4div1}{RGB}{123,50,148}
\definecolor{PRGn4div2}{RGB}{194,165,207}
\definecolor{PRGn4div3}{RGB}{166,219,160}
\definecolor{PRGn4div4}{RGB}{0,136,55}
\definecolor{PRGn6div1}{RGB}{118,42,131}
\definecolor{PRGn6div2}{RGB}{175,141,195}
\definecolor{PRGn6div3}{RGB}{231,212,232}
\definecolor{PRGn6div4}{RGB}{217,240,211}
\definecolor{PRGn6div5}{RGB}{127,191,123}
\definecolor{PRGn6div6}{RGB}{27,120,55}
\definecolor{PRGn8div1}{RGB}{118,42,131}
\definecolor{PRGn8div2}{RGB}{153,112,171}
\definecolor{PRGn8div3}{RGB}{194,165,207}
\definecolor{PRGn8div4}{RGB}{231,212,232}
\definecolor{PRGn8div5}{RGB}{217,240,211}
\definecolor{PRGn8div6}{RGB}{166,219,160}
\definecolor{PRGn8div7}{RGB}{90,174,97}
\definecolor{PRGn8div8}{RGB}{27,120,55}
\definecolor{PRGn10div1}{RGB}{64,0,75}
\definecolor{PRGn10div2}{RGB}{118,42,131}
\definecolor{PRGn10div3}{RGB}{153,112,171}
\definecolor{PRGn10div4}{RGB}{194,165,207}
\definecolor{PRGn10div5}{RGB}{231,212,232}
\definecolor{PRGn10div6}{RGB}{217,240,211}
\definecolor{PRGn10div7}{RGB}{166,219,160}
\definecolor{PRGn10div8}{RGB}{90,174,97}
\definecolor{PRGn10div9}{RGB}{27,120,55}
\definecolor{PRGn10div10}{RGB}{0,68,27}
\definecolor{PuBu3seq1}{RGB}{236,231,242}
\definecolor{PuBu3seq2}{RGB}{166,189,219}
\definecolor{PuBu3seq3}{RGB}{43,140,190}
\definecolor{PuBu5seq1}{RGB}{241,238,246}
\definecolor{PuBu5seq2}{RGB}{189,201,225}
\definecolor{PuBu5seq3}{RGB}{116,169,207}
\definecolor{PuBu5seq4}{RGB}{43,140,190}
\definecolor{PuBu5seq5}{RGB}{4,90,141}
\definecolor{PuBu7seq1}{RGB}{241,238,246}
\definecolor{PuBu7seq2}{RGB}{208,209,230}
\definecolor{PuBu7seq3}{RGB}{166,189,219}
\definecolor{PuBu7seq4}{RGB}{116,169,207}
\definecolor{PuBu7seq5}{RGB}{54,144,192}
\definecolor{PuBu7seq6}{RGB}{5,112,176}
\definecolor{PuBu7seq7}{RGB}{3,78,123}
\definecolor{PuBu9seq1}{RGB}{255,247,251}
\definecolor{PuBu9seq2}{RGB}{236,231,242}
\definecolor{PuBu9seq3}{RGB}{208,209,230}
\definecolor{PuBu9seq4}{RGB}{166,189,219}
\definecolor{PuBu9seq5}{RGB}{116,169,207}
\definecolor{PuBu9seq6}{RGB}{54,144,192}
\definecolor{PuBu9seq7}{RGB}{5,112,176}
\definecolor{PuBu9seq8}{RGB}{4,90,141}
\definecolor{PuBu9seq9}{RGB}{2,56,88}
\definecolor{PuBuGn4seq1}{RGB}{246,239,247}
\definecolor{PuBuGn4seq2}{RGB}{189,201,225}
\definecolor{PuBuGn4seq3}{RGB}{103,169,207}
\definecolor{PuBuGn4seq4}{RGB}{2,129,138}
\definecolor{PuBuGn6seq1}{RGB}{246,239,247}
\definecolor{PuBuGn6seq2}{RGB}{208,209,230}
\definecolor{PuBuGn6seq3}{RGB}{166,189,219}
\definecolor{PuBuGn6seq4}{RGB}{103,169,207}
\definecolor{PuBuGn6seq5}{RGB}{28,144,153}
\definecolor{PuBuGn6seq6}{RGB}{1,108,89}
\definecolor{PuBuGn8seq1}{RGB}{255,247,251}
\definecolor{PuBuGn8seq2}{RGB}{236,226,240}
\definecolor{PuBuGn8seq3}{RGB}{208,209,230}
\definecolor{PuBuGn8seq4}{RGB}{166,189,219}
\definecolor{PuBuGn8seq5}{RGB}{103,169,207}
\definecolor{PuBuGn8seq6}{RGB}{54,144,192}
\definecolor{PuBuGn8seq7}{RGB}{2,129,138}
\definecolor{PuBuGn8seq8}{RGB}{1,100,80}
\definecolor{PuOr3div1}{RGB}{241,163,64}
\definecolor{PuOr3div2}{RGB}{247,247,247}
\definecolor{PuOr3div3}{RGB}{153,142,195}
\definecolor{PuOr5div1}{RGB}{230,97,1}
\definecolor{PuOr5div2}{RGB}{253,184,99}
\definecolor{PuOr5div3}{RGB}{247,247,247}
\definecolor{PuOr5div4}{RGB}{178,171,210}
\definecolor{PuOr5div5}{RGB}{94,60,153}
\definecolor{PuOr7div1}{RGB}{179,88,6}
\definecolor{PuOr7div2}{RGB}{241,163,64}
\definecolor{PuOr7div3}{RGB}{254,224,182}
\definecolor{PuOr7div4}{RGB}{247,247,247}
\definecolor{PuOr7div5}{RGB}{216,218,235}
\definecolor{PuOr7div6}{RGB}{153,142,195}
\definecolor{PuOr7div7}{RGB}{84,39,136}
\definecolor{PuOr9div1}{RGB}{179,88,6}
\definecolor{PuOr9div2}{RGB}{224,130,20}
\definecolor{PuOr9div3}{RGB}{253,184,99}
\definecolor{PuOr9div4}{RGB}{254,224,182}
\definecolor{PuOr9div5}{RGB}{247,247,247}
\definecolor{PuOr9div6}{RGB}{216,218,235}
\definecolor{PuOr9div7}{RGB}{178,171,210}
\definecolor{PuOr9div8}{RGB}{128,115,172}
\definecolor{PuOr9div9}{RGB}{84,39,136}
\definecolor{PuOr11div1}{RGB}{127,59,8}
\definecolor{PuOr11div2}{RGB}{179,88,6}
\definecolor{PuOr11div3}{RGB}{224,130,20}
\definecolor{PuOr11div4}{RGB}{253,184,99}
\definecolor{PuOr11div5}{RGB}{254,224,182}
\definecolor{PuOr11div6}{RGB}{247,247,247}
\definecolor{PuOr11div7}{RGB}{216,218,235}
\definecolor{PuOr11div8}{RGB}{178,171,210}
\definecolor{PuOr11div9}{RGB}{128,115,172}
\definecolor{PuOr11div10}{RGB}{84,39,136}
\definecolor{PuOr11div11}{RGB}{45,0,75}
\definecolor{PuRd4seq1}{RGB}{241,238,246}
\definecolor{PuRd4seq2}{RGB}{215,181,216}
\definecolor{PuRd4seq3}{RGB}{223,101,176}
\definecolor{PuRd4seq4}{RGB}{206,18,86}
\definecolor{PuRd6seq1}{RGB}{241,238,246}
\definecolor{PuRd6seq2}{RGB}{212,185,218}
\definecolor{PuRd6seq3}{RGB}{201,148,199}
\definecolor{PuRd6seq4}{RGB}{223,101,176}
\definecolor{PuRd6seq5}{RGB}{221,28,119}
\definecolor{PuRd6seq6}{RGB}{152,0,67}
\definecolor{PuRd8seq1}{RGB}{247,244,249}
\definecolor{PuRd8seq2}{RGB}{231,225,239}
\definecolor{PuRd8seq3}{RGB}{212,185,218}
\definecolor{PuRd8seq4}{RGB}{201,148,199}
\definecolor{PuRd8seq5}{RGB}{223,101,176}
\definecolor{PuRd8seq6}{RGB}{231,41,138}
\definecolor{PuRd8seq7}{RGB}{206,18,86}
\definecolor{PuRd8seq8}{RGB}{145,0,63}
\definecolor{Purples3seq1}{RGB}{239,237,245}
\definecolor{Purples3seq2}{RGB}{188,189,220}
\definecolor{Purples3seq3}{RGB}{117,107,177}
\definecolor{Purples5seq1}{RGB}{242,240,247}
\definecolor{Purples5seq2}{RGB}{203,201,226}
\definecolor{Purples5seq3}{RGB}{158,154,200}
\definecolor{Purples5seq4}{RGB}{117,107,177}
\definecolor{Purples5seq5}{RGB}{84,39,143}
\definecolor{Purples7seq1}{RGB}{242,240,247}
\definecolor{Purples7seq2}{RGB}{218,218,235}
\definecolor{Purples7seq3}{RGB}{188,189,220}
\definecolor{Purples7seq4}{RGB}{158,154,200}
\definecolor{Purples7seq5}{RGB}{128,125,186}
\definecolor{Purples7seq6}{RGB}{106,81,163}
\definecolor{Purples7seq7}{RGB}{74,20,134}
\definecolor{Purples9seq1}{RGB}{252,251,253}
\definecolor{Purples9seq2}{RGB}{239,237,245}
\definecolor{Purples9seq3}{RGB}{218,218,235}
\definecolor{Purples9seq4}{RGB}{188,189,220}
\definecolor{Purples9seq5}{RGB}{158,154,200}
\definecolor{Purples9seq6}{RGB}{128,125,186}
\definecolor{Purples9seq7}{RGB}{106,81,163}
\definecolor{Purples9seq8}{RGB}{84,39,143}
\definecolor{Purples9seq9}{RGB}{63,0,125}
\definecolor{RdBu4div1}{RGB}{202,0,32}
\definecolor{RdBu4div2}{RGB}{244,165,130}
\definecolor{RdBu4div3}{RGB}{146,197,222}
\definecolor{RdBu4div4}{RGB}{5,113,176}
\definecolor{RdBu6div1}{RGB}{178,24,43}
\definecolor{RdBu6div2}{RGB}{239,138,98}
\definecolor{RdBu6div3}{RGB}{253,219,199}
\definecolor{RdBu6div4}{RGB}{209,229,240}
\definecolor{RdBu6div5}{RGB}{103,169,207}
\definecolor{RdBu6div6}{RGB}{33,102,172}
\definecolor{RdBu8div1}{RGB}{178,24,43}
\definecolor{RdBu8div2}{RGB}{214,96,77}
\definecolor{RdBu8div3}{RGB}{244,165,130}
\definecolor{RdBu8div4}{RGB}{253,219,199}
\definecolor{RdBu8div5}{RGB}{209,229,240}
\definecolor{RdBu8div6}{RGB}{146,197,222}
\definecolor{RdBu8div7}{RGB}{67,147,195}
\definecolor{RdBu8div8}{RGB}{33,102,172}
\definecolor{RdBu10div1}{RGB}{103,0,31}
\definecolor{RdBu10div2}{RGB}{178,24,43}
\definecolor{RdBu10div3}{RGB}{214,96,77}
\definecolor{RdBu10div4}{RGB}{244,165,130}
\definecolor{RdBu10div5}{RGB}{253,219,199}
\definecolor{RdBu10div6}{RGB}{209,229,240}
\definecolor{RdBu10div7}{RGB}{146,197,222}
\definecolor{RdBu10div8}{RGB}{67,147,195}
\definecolor{RdBu10div9}{RGB}{33,102,172}
\definecolor{RdBu10div10}{RGB}{5,48,97}
\definecolor{RdGy3div1}{RGB}{239,138,98}
\definecolor{RdGy3div2}{RGB}{255,255,255}
\definecolor{RdGy3div3}{RGB}{153,153,153}
\definecolor{RdGy5div1}{RGB}{202,0,32}
\definecolor{RdGy5div2}{RGB}{244,165,130}
\definecolor{RdGy5div3}{RGB}{255,255,255}
\definecolor{RdGy5div4}{RGB}{186,186,186}
\definecolor{RdGy5div5}{RGB}{64,64,64}
\definecolor{RdGy7div1}{RGB}{178,24,43}
\definecolor{RdGy7div2}{RGB}{239,138,98}
\definecolor{RdGy7div3}{RGB}{253,219,199}
\definecolor{RdGy7div4}{RGB}{255,255,255}
\definecolor{RdGy7div5}{RGB}{224,224,224}
\definecolor{RdGy7div6}{RGB}{153,153,153}
\definecolor{RdGy7div7}{RGB}{77,77,77}
\definecolor{RdGy9div1}{RGB}{178,24,43}
\definecolor{RdGy9div2}{RGB}{214,96,77}
\definecolor{RdGy9div3}{RGB}{244,165,130}
\definecolor{RdGy9div4}{RGB}{253,219,199}
\definecolor{RdGy9div5}{RGB}{255,255,255}
\definecolor{RdGy9div6}{RGB}{224,224,224}
\definecolor{RdGy9div7}{RGB}{186,186,186}
\definecolor{RdGy9div8}{RGB}{135,135,135}
\definecolor{RdGy9div9}{RGB}{77,77,77}
\definecolor{RdGy11div1}{RGB}{103,0,31}
\definecolor{RdGy11div2}{RGB}{178,24,43}
\definecolor{RdGy11div3}{RGB}{214,96,77}
\definecolor{RdGy11div4}{RGB}{244,165,130}
\definecolor{RdGy11div5}{RGB}{253,219,199}
\definecolor{RdGy11div6}{RGB}{255,255,255}
\definecolor{RdGy11div7}{RGB}{224,224,224}
\definecolor{RdGy11div8}{RGB}{186,186,186}
\definecolor{RdGy11div9}{RGB}{135,135,135}
\definecolor{RdGy11div10}{RGB}{77,77,77}
\definecolor{RdGy11div11}{RGB}{26,26,26}
\definecolor{RdPu4seq1}{RGB}{254,235,226}
\definecolor{RdPu4seq2}{RGB}{251,180,185}
\definecolor{RdPu4seq3}{RGB}{247,104,161}
\definecolor{RdPu4seq4}{RGB}{174,1,126}
\definecolor{RdPu6seq1}{RGB}{254,235,226}
\definecolor{RdPu6seq2}{RGB}{252,197,192}
\definecolor{RdPu6seq3}{RGB}{250,159,181}
\definecolor{RdPu6seq4}{RGB}{247,104,161}
\definecolor{RdPu6seq5}{RGB}{197,27,138}
\definecolor{RdPu6seq6}{RGB}{122,1,119}
\definecolor{RdPu8seq1}{RGB}{255,247,243}
\definecolor{RdPu8seq2}{RGB}{253,224,221}
\definecolor{RdPu8seq3}{RGB}{252,197,192}
\definecolor{RdPu8seq4}{RGB}{250,159,181}
\definecolor{RdPu8seq5}{RGB}{247,104,161}
\definecolor{RdPu8seq6}{RGB}{221,52,151}
\definecolor{RdPu8seq7}{RGB}{174,1,126}
\definecolor{RdPu8seq8}{RGB}{122,1,119}

%EDIT: Added number of classes
\definecolor{Reds3seq1}{RGB}{254,224,210}
\definecolor{Reds3seq2}{RGB}{252,146,114}
\definecolor{Reds3seq3}{RGB}{222,45,38}

\definecolor{Reds4seq1}{RGB}{254,229,217}
\definecolor{Reds4seq2}{RGB}{252,174,145}
\definecolor{Reds4seq3}{RGB}{251,106,74}
\definecolor{Reds4seq4}{RGB}{203,24,29}

\definecolor{Reds5seq1}{RGB}{254,229,217}
\definecolor{Reds5seq2}{RGB}{252,174,145}
\definecolor{Reds5seq3}{RGB}{251,106,74}
\definecolor{Reds5seq4}{RGB}{222,45,38}
\definecolor{Reds5seq5}{RGB}{165,15,21}

\definecolor{Reds6seq1}{RGB}{254,229,217}
\definecolor{Reds6seq2}{RGB}{252,187,161}
\definecolor{Reds6seq3}{RGB}{252,146,114}
\definecolor{Reds6seq4}{RGB}{251,106,74}
\definecolor{Reds6seq5}{RGB}{222,45,38}
\definecolor{Reds6seq6}{RGB}{165,15,21}

\definecolor{Reds7seq1}{RGB}{254,229,217}
\definecolor{Reds7seq2}{RGB}{252,187,161}
\definecolor{Reds7seq3}{RGB}{252,146,114}
\definecolor{Reds7seq4}{RGB}{251,106,74}
\definecolor{Reds7seq5}{RGB}{239,59,44}
\definecolor{Reds7seq6}{RGB}{203,24,29}
\definecolor{Reds7seq7}{RGB}{153,0,13}

\definecolor{Reds8seq1}{RGB}{255,245,240}
\definecolor{Reds8seq2}{RGB}{254,224,210}
\definecolor{Reds8seq3}{RGB}{252,187,161}
\definecolor{Reds8seq4}{RGB}{252,146,114}
\definecolor{Reds8seq5}{RGB}{251,106,74}
\definecolor{Reds8seq6}{RGB}{239,59,44}
\definecolor{Reds8seq7}{RGB}{203,24,29}
\definecolor{Reds8seq8}{RGB}{153,0,13}

\definecolor{Reds9seq1}{RGB}{255,245,240}
\definecolor{Reds9seq2}{RGB}{254,224,210}
\definecolor{Reds9seq3}{RGB}{252,187,161}
\definecolor{Reds9seq4}{RGB}{252,146,114}
\definecolor{Reds9seq5}{RGB}{251,106,74}
\definecolor{Reds9seq6}{RGB}{239,59,44}
\definecolor{Reds9seq7}{RGB}{203,24,29}
\definecolor{Reds9seq8}{RGB}{165,15,21}
\definecolor{Reds9seq9}{RGB}{103,0,13}

\definecolor{RdYlBu3div1}{RGB}{252,141,89}
\definecolor{RdYlBu3div2}{RGB}{255,255,191}
\definecolor{RdYlBu3div3}{RGB}{145,191,219}

\definecolor{RdYlBu4div1}{RGB}{215,25,28}
\definecolor{RdYlBu4div2}{RGB}{253,174,97}
\definecolor{RdYlBu4div3}{RGB}{171,217,233}
\definecolor{RdYlBu4div4}{RGB}{44,123,182}

\definecolor{RdYlBu5div1}{RGB}{215,25,28}
\definecolor{RdYlBu5div2}{RGB}{253,174,97}
\definecolor{RdYlBu5div3}{RGB}{255,255,191}
\definecolor{RdYlBu5div4}{RGB}{171,217,233}
\definecolor{RdYlBu5div5}{RGB}{44,123,182}

\definecolor{RdYlBu6div1}{RGB}{215,48,39}
\definecolor{RdYlBu6div2}{RGB}{252,141,89}
\definecolor{RdYlBu6div3}{RGB}{254,224,144}
\definecolor{RdYlBu6div4}{RGB}{224,243,248}
\definecolor{RdYlBu6div5}{RGB}{145,191,219}
\definecolor{RdYlBu6div6}{RGB}{69,117,180}

\definecolor{RdYlBu7div1}{RGB}{215,48,39}
\definecolor{RdYlBu7div2}{RGB}{252,141,89}
\definecolor{RdYlBu7div3}{RGB}{254,224,144}
\definecolor{RdYlBu7div4}{RGB}{255,255,191}
\definecolor{RdYlBu7div5}{RGB}{224,243,248}
\definecolor{RdYlBu7div6}{RGB}{145,191,219}
\definecolor{RdYlBu7div7}{RGB}{69,117,180}

\definecolor{RdYlBu8div1}{RGB}{215,48,39}
\definecolor{RdYlBu8div2}{RGB}{244,109,67}
\definecolor{RdYlBu8div3}{RGB}{253,174,97}
\definecolor{RdYlBu8div4}{RGB}{254,224,144}
\definecolor{RdYlBu8div5}{RGB}{224,243,248}
\definecolor{RdYlBu8div6}{RGB}{171,217,233}
\definecolor{RdYlBu8div7}{RGB}{116,173,209}
\definecolor{RdYlBu8div8}{RGB}{69,117,180}

\definecolor{RdYlBu9div1}{RGB}{215,48,39}
\definecolor{RdYlBu9div2}{RGB}{244,109,67}
\definecolor{RdYlBu9div3}{RGB}{253,174,97}
\definecolor{RdYlBu9div4}{RGB}{254,224,144}
\definecolor{RdYlBu9div5}{RGB}{255,255,191}
\definecolor{RdYlBu9div6}{RGB}{224,243,248}
\definecolor{RdYlBu9div7}{RGB}{171,217,233}
\definecolor{RdYlBu9div8}{RGB}{116,173,209}
\definecolor{RdYlBu9div9}{RGB}{69,117,180}

\definecolor{RdYlBu10div1}{RGB}{165,0,38}
\definecolor{RdYlBu10div2}{RGB}{215,48,39}
\definecolor{RdYlBu10div3}{RGB}{244,109,67}
\definecolor{RdYlBu10div4}{RGB}{253,174,97}
\definecolor{RdYlBu10div5}{RGB}{254,224,144}
\definecolor{RdYlBu10div6}{RGB}{224,243,248}
\definecolor{RdYlBu10div7}{RGB}{171,217,233}
\definecolor{RdYlBu10div8}{RGB}{116,173,209}
\definecolor{RdYlBu10div9}{RGB}{69,117,180}
\definecolor{RdYlBu10div10}{RGB}{49,54,149}


\definecolor{RdYlGn3div1}{RGB}{252,141,89}
\definecolor{RdYlGn3div2}{RGB}{255,255,191}
\definecolor{RdYlGn3div3}{RGB}{145,207,96}

\definecolor{RdYlGn4div1}{RGB}{215,25,28}
\definecolor{RdYlGn4div2}{RGB}{253,174,97}
\definecolor{RdYlGn4div3}{RGB}{166,217,106}
\definecolor{RdYlGn4div4}{RGB}{26,150,65}

\definecolor{RdYlGn5div1}{RGB}{215,25,28}
\definecolor{RdYlGn5div2}{RGB}{253,174,97}
\definecolor{RdYlGn5div3}{RGB}{255,255,191}
\definecolor{RdYlGn5div4}{RGB}{166,217,106}
\definecolor{RdYlGn5div5}{RGB}{26,150,65}

\definecolor{RdYlGn6div1}{RGB}{215,48,39}
\definecolor{RdYlGn6div2}{RGB}{252,141,89}
\definecolor{RdYlGn6div3}{RGB}{254,224,139}
\definecolor{RdYlGn6div4}{RGB}{217,239,139}
\definecolor{RdYlGn6div5}{RGB}{145,207,96}
\definecolor{RdYlGn6div6}{RGB}{26,152,80}

\definecolor{RdYlGn7div1}{RGB}{215,48,39}
\definecolor{RdYlGn7div2}{RGB}{252,141,89}
\definecolor{RdYlGn7div3}{RGB}{254,224,139}
\definecolor{RdYlGn7div4}{RGB}{255,255,191}
\definecolor{RdYlGn7div5}{RGB}{217,239,139}
\definecolor{RdYlGn7div6}{RGB}{145,207,96}
\definecolor{RdYlGn7div7}{RGB}{26,152,80}

\definecolor{RdYlGn8div1}{RGB}{215,48,39}
\definecolor{RdYlGn8div2}{RGB}{244,109,67}
\definecolor{RdYlGn8div3}{RGB}{253,174,97}
\definecolor{RdYlGn8div4}{RGB}{254,224,139}
\definecolor{RdYlGn8div5}{RGB}{217,239,139}
\definecolor{RdYlGn8div6}{RGB}{166,217,106}
\definecolor{RdYlGn8div7}{RGB}{102,189,99}
\definecolor{RdYlGn8div8}{RGB}{26,152,80}

\definecolor{RdYlGn9div1}{RGB}{215,48,39}
\definecolor{RdYlGn9div2}{RGB}{244,109,67}
\definecolor{RdYlGn9div3}{RGB}{253,174,97}
\definecolor{RdYlGn9div4}{RGB}{254,224,139}
\definecolor{RdYlGn9div5}{RGB}{255,255,191}
\definecolor{RdYlGn9div6}{RGB}{217,239,139}
\definecolor{RdYlGn9div7}{RGB}{166,217,106}
\definecolor{RdYlGn9div8}{RGB}{102,189,99}
\definecolor{RdYlGn9div9}{RGB}{26,152,80}

\definecolor{RdYlGn10div1}{RGB}{165,0,38}
\definecolor{RdYlGn10div2}{RGB}{215,48,39}
\definecolor{RdYlGn10div3}{RGB}{244,109,67}
\definecolor{RdYlGn10div4}{RGB}{253,174,97}
\definecolor{RdYlGn10div5}{RGB}{254,224,139}
\definecolor{RdYlGn10div6}{RGB}{217,239,139}
\definecolor{RdYlGn10div7}{RGB}{166,217,106}
\definecolor{RdYlGn10div8}{RGB}{102,189,99}
\definecolor{RdYlGn10div9}{RGB}{26,152,80}
\definecolor{RdYlGn10div10}{RGB}{0,104,55}

\definecolor{RdYlGn11div1}{RGB}{165,0,38}
\definecolor{RdYlGn11div2}{RGB}{215,48,39}
\definecolor{RdYlGn11div3}{RGB}{244,109,67}
\definecolor{RdYlGn11div4}{RGB}{253,174,97}
\definecolor{RdYlGn11div5}{RGB}{254,224,139}
\definecolor{RdYlGn11div6}{RGB}{255,255,191}
\definecolor{RdYlGn11div7}{RGB}{217,239,139}
\definecolor{RdYlGn11div8}{RGB}{166,217,106}
\definecolor{RdYlGn11div9}{RGB}{102,189,99}
\definecolor{RdYlGn11div10}{RGB}{26,152,80}
\definecolor{RdYlGn11div11}{RGB}{0,104,55}
%END EDIT

\definecolor{Set14qual1}{RGB}{228,26,28}
\definecolor{Set14qual2}{RGB}{55,126,184}
\definecolor{Set14qual3}{RGB}{77,175,74}
\definecolor{Set14qual4}{RGB}{152,78,163}
\definecolor{Set16qual1}{RGB}{228,26,28}
\definecolor{Set16qual2}{RGB}{55,126,184}
\definecolor{Set16qual3}{RGB}{77,175,74}
\definecolor{Set16qual4}{RGB}{152,78,163}
\definecolor{Set16qual5}{RGB}{255,127,0}
\definecolor{Set16qual6}{RGB}{255,255,51}
\definecolor{Set18qual1}{RGB}{228,26,28}
\definecolor{Set18qual2}{RGB}{55,126,184}
\definecolor{Set18qual3}{RGB}{77,175,74}
\definecolor{Set18qual4}{RGB}{152,78,163}
\definecolor{Set18qual5}{RGB}{255,127,0}
\definecolor{Set18qual6}{RGB}{255,255,51}
\definecolor{Set18qual7}{RGB}{166,86,40}
\definecolor{Set18qual8}{RGB}{247,129,191}
\definecolor{Set23qual1}{RGB}{102,194,165}
\definecolor{Set23qual2}{RGB}{252,141,98}
\definecolor{Set23qual3}{RGB}{141,160,203}
\definecolor{Set25qual1}{RGB}{102,194,165}
\definecolor{Set25qual2}{RGB}{252,141,98}
\definecolor{Set25qual3}{RGB}{141,160,203}
\definecolor{Set25qual4}{RGB}{231,138,195}
\definecolor{Set25qual5}{RGB}{166,216,84}
\definecolor{Set27qual1}{RGB}{102,194,165}
\definecolor{Set27qual2}{RGB}{252,141,98}
\definecolor{Set27qual3}{RGB}{141,160,203}
\definecolor{Set27qual4}{RGB}{231,138,195}
\definecolor{Set27qual5}{RGB}{166,216,84}
\definecolor{Set27qual6}{RGB}{255,217,47}
\definecolor{Set27qual7}{RGB}{229,196,148}
\definecolor{Set33qual1}{RGB}{141,211,199}
\definecolor{Set33qual2}{RGB}{255,255,179}
\definecolor{Set33qual3}{RGB}{190,186,218}
\definecolor{Set35qual1}{RGB}{141,211,199}
\definecolor{Set35qual2}{RGB}{255,255,179}
\definecolor{Set35qual3}{RGB}{190,186,218}
\definecolor{Set35qual4}{RGB}{251,128,114}
\definecolor{Set35qual5}{RGB}{128,177,211}
\definecolor{Set37qual1}{RGB}{141,211,199}
\definecolor{Set37qual2}{RGB}{255,255,179}
\definecolor{Set37qual3}{RGB}{190,186,218}
\definecolor{Set37qual4}{RGB}{251,128,114}
\definecolor{Set37qual5}{RGB}{128,177,211}
\definecolor{Set37qual6}{RGB}{253,180,98}
\definecolor{Set37qual7}{RGB}{179,222,105}
\definecolor{Set39qual1}{RGB}{141,211,199}
\definecolor{Set39qual2}{RGB}{255,255,179}
\definecolor{Set39qual3}{RGB}{190,186,218}
\definecolor{Set39qual4}{RGB}{251,128,114}
\definecolor{Set39qual5}{RGB}{128,177,211}
\definecolor{Set39qual6}{RGB}{253,180,98}
\definecolor{Set39qual7}{RGB}{179,222,105}
\definecolor{Set39qual8}{RGB}{252,205,229}
\definecolor{Set39qual9}{RGB}{217,217,217}
\definecolor{Set311qual1}{RGB}{141,211,199}
\definecolor{Set311qual2}{RGB}{255,255,179}
\definecolor{Set311qual3}{RGB}{190,186,218}
\definecolor{Set311qual4}{RGB}{251,128,114}
\definecolor{Set311qual5}{RGB}{128,177,211}
\definecolor{Set311qual6}{RGB}{253,180,98}
\definecolor{Set311qual7}{RGB}{179,222,105}
\definecolor{Set311qual8}{RGB}{252,205,229}
\definecolor{Set311qual9}{RGB}{217,217,217}
\definecolor{Set311qual10}{RGB}{188,128,189}
\definecolor{Set311qual11}{RGB}{204,235,197}
\definecolor{Spectral3div1}{RGB}{252,141,89}
\definecolor{Spectral3div2}{RGB}{255,255,191}
\definecolor{Spectral3div3}{RGB}{153,213,148}
\definecolor{Spectral5div1}{RGB}{215,25,28}
\definecolor{Spectral5div2}{RGB}{253,174,97}
\definecolor{Spectral5div3}{RGB}{255,255,191}
\definecolor{Spectral5div4}{RGB}{171,221,164}
\definecolor{Spectral5div5}{RGB}{43,131,186}
\definecolor{Spectral7div1}{RGB}{213,62,79}
\definecolor{Spectral7div2}{RGB}{252,141,89}
\definecolor{Spectral7div3}{RGB}{254,224,139}
\definecolor{Spectral7div4}{RGB}{255,255,191}
\definecolor{Spectral7div5}{RGB}{230,245,152}
\definecolor{Spectral7div6}{RGB}{153,213,148}
\definecolor{Spectral7div7}{RGB}{50,136,189}
\definecolor{Spectral9div1}{RGB}{213,62,79}
\definecolor{Spectral9div2}{RGB}{244,109,67}
\definecolor{Spectral9div3}{RGB}{253,174,97}
\definecolor{Spectral9div4}{RGB}{254,224,139}
\definecolor{Spectral9div5}{RGB}{255,255,191}
\definecolor{Spectral9div6}{RGB}{230,245,152}
\definecolor{Spectral9div7}{RGB}{171,221,164}
\definecolor{Spectral9div8}{RGB}{102,194,165}
\definecolor{Spectral9div9}{RGB}{50,136,189}
\definecolor{Spectral11div1}{RGB}{158,1,66}
\definecolor{Spectral11div2}{RGB}{213,62,79}
\definecolor{Spectral11div3}{RGB}{244,109,67}
\definecolor{Spectral11div4}{RGB}{253,174,97}
\definecolor{Spectral11div5}{RGB}{254,224,139}
\definecolor{Spectral11div6}{RGB}{255,255,191}
\definecolor{Spectral11div7}{RGB}{230,245,152}
\definecolor{Spectral11div8}{RGB}{171,221,164}
\definecolor{Spectral11div9}{RGB}{102,194,165}
\definecolor{Spectral11div10}{RGB}{50,136,189}
\definecolor{Spectral11div11}{RGB}{94,79,162}
\definecolor{YlGn4seq1}{RGB}{255,255,204}
\definecolor{YlGn4seq2}{RGB}{194,230,153}
\definecolor{YlGn4seq3}{RGB}{120,198,121}
\definecolor{YlGn4seq4}{RGB}{35,132,67}
\definecolor{YlGn6seq1}{RGB}{255,255,204}
\definecolor{YlGn6seq2}{RGB}{217,240,163}
\definecolor{YlGn6seq3}{RGB}{173,221,142}
\definecolor{YlGn6seq4}{RGB}{120,198,121}
\definecolor{YlGn6seq5}{RGB}{49,163,84}
\definecolor{YlGn6seq6}{RGB}{0,104,55}
\definecolor{YlGn8seq1}{RGB}{255,255,229}
\definecolor{YlGn8seq2}{RGB}{247,252,185}
\definecolor{YlGn8seq3}{RGB}{217,240,163}
\definecolor{YlGn8seq4}{RGB}{173,221,142}
\definecolor{YlGn8seq5}{RGB}{120,198,121}
\definecolor{YlGn8seq6}{RGB}{65,171,93}
\definecolor{YlGn8seq7}{RGB}{35,132,67}
\definecolor{YlGn8seq8}{RGB}{0,90,50}
\definecolor{YlGnBu3seq1}{RGB}{237,248,177}
\definecolor{YlGnBu3seq2}{RGB}{127,205,187}
\definecolor{YlGnBu3seq3}{RGB}{44,127,184}
\definecolor{YlGnBu5seq1}{RGB}{255,255,204}
\definecolor{YlGnBu5seq2}{RGB}{161,218,180}
\definecolor{YlGnBu5seq3}{RGB}{65,182,196}
\definecolor{YlGnBu5seq4}{RGB}{44,127,184}
\definecolor{YlGnBu5seq5}{RGB}{37,52,148}
\definecolor{YlGnBu7seq1}{RGB}{255,255,204}
\definecolor{YlGnBu7seq2}{RGB}{199,233,180}
\definecolor{YlGnBu7seq3}{RGB}{127,205,187}
\definecolor{YlGnBu7seq4}{RGB}{65,182,196}
\definecolor{YlGnBu7seq5}{RGB}{29,145,192}
\definecolor{YlGnBu7seq6}{RGB}{34,94,168}
\definecolor{YlGnBu7seq7}{RGB}{12,44,132}
\definecolor{YlGnBu9seq1}{RGB}{255,255,217}
\definecolor{YlGnBu9seq2}{RGB}{237,248,177}
\definecolor{YlGnBu9seq3}{RGB}{199,233,180}
\definecolor{YlGnBu9seq4}{RGB}{127,205,187}
\definecolor{YlGnBu9seq5}{RGB}{65,182,196}
\definecolor{YlGnBu9seq6}{RGB}{29,145,192}
\definecolor{YlGnBu9seq7}{RGB}{34,94,168}
\definecolor{YlGnBu9seq8}{RGB}{37,52,148}
\definecolor{YlGnBu9seq9}{RGB}{8,29,88}
\definecolor{YlOrBr4seq1}{RGB}{255,255,212}
\definecolor{YlOrBr4seq2}{RGB}{254,217,142}
\definecolor{YlOrBr4seq3}{RGB}{254,153,41}
\definecolor{YlOrBr4seq4}{RGB}{204,76,2}
\definecolor{YlOrBr6seq1}{RGB}{255,255,212}
\definecolor{YlOrBr6seq2}{RGB}{254,227,145}
\definecolor{YlOrBr6seq3}{RGB}{254,196,79}
\definecolor{YlOrBr6seq4}{RGB}{254,153,41}
\definecolor{YlOrBr6seq5}{RGB}{217,95,14}
\definecolor{YlOrBr6seq6}{RGB}{153,52,4}
\definecolor{YlOrBr8seq1}{RGB}{255,255,229}
\definecolor{YlOrBr8seq2}{RGB}{255,247,188}
\definecolor{YlOrBr8seq3}{RGB}{254,227,145}
\definecolor{YlOrBr8seq4}{RGB}{254,196,79}
\definecolor{YlOrBr8seq5}{RGB}{254,153,41}
\definecolor{YlOrBr8seq6}{RGB}{236,112,20}
\definecolor{YlOrBr8seq7}{RGB}{204,76,2}
\definecolor{YlOrBr8seq8}{RGB}{140,45,4}
\definecolor{YlOrRd3seq1}{RGB}{255,237,160}
\definecolor{YlOrRd3seq2}{RGB}{254,178,76}
\definecolor{YlOrRd3seq3}{RGB}{240,59,32}
\definecolor{YlOrRd5seq1}{RGB}{255,255,178}
\definecolor{YlOrRd5seq2}{RGB}{254,204,92}
\definecolor{YlOrRd5seq3}{RGB}{253,141,60}
\definecolor{YlOrRd5seq4}{RGB}{240,59,32}
\definecolor{YlOrRd5seq5}{RGB}{189,0,38}
\definecolor{YlOrRd7seq1}{RGB}{255,255,178}
\definecolor{YlOrRd7seq2}{RGB}{254,217,118}
\definecolor{YlOrRd7seq3}{RGB}{254,178,76}
\definecolor{YlOrRd7seq4}{RGB}{253,141,60}
\definecolor{YlOrRd7seq5}{RGB}{252,78,42}
\definecolor{YlOrRd7seq6}{RGB}{227,26,28}
\definecolor{YlOrRd7seq7}{RGB}{177,0,38}
\definecolor{YlOrRd9seq1}{RGB}{255,255,204}
\definecolor{YlOrRd9seq2}{RGB}{255,237,160}
\definecolor{YlOrRd9seq3}{RGB}{254,217,118}
\definecolor{YlOrRd9seq4}{RGB}{254,178,76}
\definecolor{YlOrRd9seq5}{RGB}{253,141,60}
\definecolor{YlOrRd9seq6}{RGB}{252,78,42}
\definecolor{YlOrRd9seq7}{RGB}{227,26,28}
\definecolor{YlOrRd9seq8}{RGB}{189,0,38}
\definecolor{YlOrRd9seq9}{RGB}{128,0,38}
\pgfplotsset{/pgfplots/colormap={Accent3qual}{
	rgb255=(127,201,127) 
	rgb255=(190,174,212) 
	rgb255=(253,192,134) 
}}
\pgfplotsset{/pgfplots/colormap={Accent5qual}{
	rgb255=(127,201,127) 
	rgb255=(190,174,212) 
	rgb255=(253,192,134) 
	rgb255=(255,255,153) 
	rgb255=(56,108,176) 
}}
\pgfplotsset{/pgfplots/colormap={Accent7qual}{
	rgb255=(127,201,127) 
	rgb255=(190,174,212) 
	rgb255=(253,192,134) 
	rgb255=(255,255,153) 
	rgb255=(56,108,176) 
	rgb255=(240,2,127) 
	rgb255=(191,91,23) 
}}

%EDIT: Added number of classes
\pgfplotsset{/pgfplots/colormap={BluesSeq}{
	rgb255=(239,243,255)
	rgb255=(189,215,231)
	rgb255=(107,174,214)
	rgb255=(49,130,189)
	rgb255=(8,81,156)
}}

\pgfplotsset{/pgfplots/colormap={Blues3seq}{
	rgb255=(222,235,247) 
	rgb255=(158,202,225) 
	rgb255=(49,130,189) 
}}
\pgfplotsset{/pgfplots/colormap={Blues5seq}{
	rgb255=(239,243,255) 
	rgb255=(189,215,231) 
	rgb255=(107,174,214) 
	rgb255=(49,130,189) 
	rgb255=(8,81,156) 
}}
\pgfplotsset{/pgfplots/colormap={Blues7seq}{
	rgb255=(239,243,255) 
	rgb255=(198,219,239) 
	rgb255=(158,202,225) 
	rgb255=(107,174,214) 
	rgb255=(66,146,198) 
	rgb255=(33,113,181) 
	rgb255=(8,69,148) 
}}
\pgfplotsset{/pgfplots/colormap={Blues9seq}{
	rgb255=(247,251,255) 
	rgb255=(222,235,247) 
	rgb255=(198,219,239) 
	rgb255=(158,202,225) 
	rgb255=(107,174,214) 
	rgb255=(66,146,198) 
	rgb255=(33,113,181) 
	rgb255=(8,81,156) 
	rgb255=(8,48,107) 
}}
%END EDIT

\pgfplotsset{/pgfplots/colormap={BrBG4div}{
	rgb255=(166,97,26) 
	rgb255=(223,194,125) 
	rgb255=(128,205,193) 
	rgb255=(1,133,113) 
}}
\pgfplotsset{/pgfplots/colormap={BrBG6div}{
	rgb255=(140,81,10) 
	rgb255=(216,179,101) 
	rgb255=(246,232,195) 
	rgb255=(199,234,229) 
	rgb255=(90,180,172) 
	rgb255=(1,102,94) 
}}
\pgfplotsset{/pgfplots/colormap={BrBG8div}{
	rgb255=(140,81,10) 
	rgb255=(191,129,45) 
	rgb255=(223,194,125) 
	rgb255=(246,232,195) 
	rgb255=(199,234,229) 
	rgb255=(128,205,193) 
	rgb255=(53,151,143) 
	rgb255=(1,102,94) 
}}
\pgfplotsset{/pgfplots/colormap={BrBG10div}{
	rgb255=(84,48,5) 
	rgb255=(140,81,10) 
	rgb255=(191,129,45) 
	rgb255=(223,194,125) 
	rgb255=(246,232,195) 
	rgb255=(199,234,229) 
	rgb255=(128,205,193) 
	rgb255=(53,151,143) 
	rgb255=(1,102,94) 
	rgb255=(0,60,48) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn3seq}{
	rgb255=(229,245,249) 
	rgb255=(153,216,201) 
	rgb255=(44,162,95) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn5seq}{
	rgb255=(237,248,251) 
	rgb255=(178,226,226) 
	rgb255=(102,194,164) 
	rgb255=(44,162,95) 
	rgb255=(0,109,44) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn7seq}{
	rgb255=(237,248,251) 
	rgb255=(204,236,230) 
	rgb255=(153,216,201) 
	rgb255=(102,194,164) 
	rgb255=(65,174,118) 
	rgb255=(35,139,69) 
	rgb255=(0,88,36) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn9seq}{
	rgb255=(247,252,253) 
	rgb255=(229,245,249) 
	rgb255=(204,236,230) 
	rgb255=(153,216,201) 
	rgb255=(102,194,164) 
	rgb255=(65,174,118) 
	rgb255=(35,139,69) 
	rgb255=(0,109,44) 
	rgb255=(0,68,27) 
}}
\pgfplotsset{/pgfplots/colormap={BuPu4seq}{
	rgb255=(237,248,251) 
	rgb255=(179,205,227) 
	rgb255=(140,150,198) 
	rgb255=(136,65,157) 
}}
\pgfplotsset{/pgfplots/colormap={BuPu6seq}{
	rgb255=(237,248,251) 
	rgb255=(191,211,230) 
	rgb255=(158,188,218) 
	rgb255=(140,150,198) 
	rgb255=(136,86,167) 
	rgb255=(129,15,124) 
}}
\pgfplotsset{/pgfplots/colormap={BuPu8seq}{
	rgb255=(247,252,253) 
	rgb255=(224,236,244) 
	rgb255=(191,211,230) 
	rgb255=(158,188,218) 
	rgb255=(140,150,198) 
	rgb255=(140,107,177) 
	rgb255=(136,65,157) 
	rgb255=(110,1,107) 
}}
\pgfplotsset{/pgfplots/colormap={Dark23qual}{
	rgb255=(27,158,119) 
	rgb255=(217,95,2) 
	rgb255=(117,112,179) 
}}
\pgfplotsset{/pgfplots/colormap={Dark25qual}{
	rgb255=(27,158,119) 
	rgb255=(217,95,2) 
	rgb255=(117,112,179) 
	rgb255=(231,41,138) 
	rgb255=(102,166,30) 
}}
\pgfplotsset{/pgfplots/colormap={Dark27qual}{
	rgb255=(27,158,119) 
	rgb255=(217,95,2) 
	rgb255=(117,112,179) 
	rgb255=(231,41,138) 
	rgb255=(102,166,30) 
	rgb255=(230,171,2) 
	rgb255=(166,118,29) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu3seq}{
	rgb255=(224,243,219) 
	rgb255=(168,221,181) 
	rgb255=(67,162,202) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu5seq}{
	rgb255=(240,249,232) 
	rgb255=(186,228,188) 
	rgb255=(123,204,196) 
	rgb255=(67,162,202) 
	rgb255=(8,104,172) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu7seq}{
	rgb255=(240,249,232) 
	rgb255=(204,235,197) 
	rgb255=(168,221,181) 
	rgb255=(123,204,196) 
	rgb255=(78,179,211) 
	rgb255=(43,140,190) 
	rgb255=(8,88,158) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu9seq}{
	rgb255=(247,252,240) 
	rgb255=(224,243,219) 
	rgb255=(204,235,197) 
	rgb255=(168,221,181) 
	rgb255=(123,204,196) 
	rgb255=(78,179,211) 
	rgb255=(43,140,190) 
	rgb255=(8,104,172) 
	rgb255=(8,64,129) 
}}

%EDIT: Added number of classes
\pgfplotsset{/pgfplots/colormap={GreensSeq}{
	rgb255=(237,248,233)
	rgb255=(186,228,179)
	rgb255=(116,196,118)
	rgb255=(49,163,84)
	rgb255=(0,109,44)
}}

\pgfplotsset{/pgfplots/colormap={Greens3seq}{
	rgb255=(237,248,233)
	rgb255=(161,217,155)
	rgb255=(49,163,84)
}}
\pgfplotsset{/pgfplots/colormap={Greens4seq}{
	rgb255=(237,248,233) 
	rgb255=(186,228,179) 
	rgb255=(116,196,118) 
	rgb255=(35,139,69) 
}}
\pgfplotsset{/pgfplots/colormap={Greens6seq}{
	rgb255=(237,248,233) 
	rgb255=(199,233,192) 
	rgb255=(161,217,155) 
	rgb255=(116,196,118) 
	rgb255=(49,163,84) 
	rgb255=(0,109,44) 
}}
\pgfplotsset{/pgfplots/colormap={Greens8seq}{
	rgb255=(247,252,245) 
	rgb255=(229,245,224) 
	rgb255=(199,233,192) 
	rgb255=(161,217,155) 
	rgb255=(116,196,118) 
	rgb255=(65,171,93) 
	rgb255=(35,139,69) 
	rgb255=(0,90,50) 
}}
\pgfplotsset{/pgfplots/colormap={Greens9seq}{
	rgb255=(247,252,245)
	rgb255=(229,245,224)
	rgb255=(199,233,192)
	rgb255=(161,217,155)
	rgb255=(116,196,118)
	rgb255=(65,171,93)
	rgb255=(35,139,69)
	rgb255=(0,109,44)
	rgb255=(0,68,27)
}}
%END EDIT

\pgfplotsset{/pgfplots/colormap={Greys3seq}{
	rgb255=(240,240,240) 
	rgb255=(189,189,189) 
	rgb255=(99,99,99) 
}}
\pgfplotsset{/pgfplots/colormap={Greys5seq}{
	rgb255=(247,247,247) 
	rgb255=(204,204,204) 
	rgb255=(150,150,150) 
	rgb255=(99,99,99) 
	rgb255=(37,37,37) 
}}
\pgfplotsset{/pgfplots/colormap={Greys7seq}{
	rgb255=(247,247,247) 
	rgb255=(217,217,217) 
	rgb255=(189,189,189) 
	rgb255=(150,150,150) 
	rgb255=(115,115,115) 
	rgb255=(82,82,82) 
	rgb255=(37,37,37) 
}}
\pgfplotsset{/pgfplots/colormap={Greys9seq}{
	rgb255=(255,255,255) 
	rgb255=(240,240,240) 
	rgb255=(217,217,217) 
	rgb255=(189,189,189) 
	rgb255=(150,150,150) 
	rgb255=(115,115,115) 
	rgb255=(82,82,82) 
	rgb255=(37,37,37) 
	rgb255=(0,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={Oranges4seq}{
	rgb255=(254,237,222) 
	rgb255=(253,190,133) 
	rgb255=(253,141,60) 
	rgb255=(217,71,1) 
}}
\pgfplotsset{/pgfplots/colormap={Oranges6seq}{
	rgb255=(254,237,222) 
	rgb255=(253,208,162) 
	rgb255=(253,174,107) 
	rgb255=(253,141,60) 
	rgb255=(230,85,13) 
	rgb255=(166,54,3) 
}}
\pgfplotsset{/pgfplots/colormap={Oranges8seq}{
	rgb255=(255,245,235) 
	rgb255=(254,230,206) 
	rgb255=(253,208,162) 
	rgb255=(253,174,107) 
	rgb255=(253,141,60) 
	rgb255=(241,105,19) 
	rgb255=(217,72,1) 
	rgb255=(140,45,4) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd3seq}{
	rgb255=(254,232,200) 
	rgb255=(253,187,132) 
	rgb255=(227,74,51) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd5seq}{
	rgb255=(254,240,217) 
	rgb255=(253,204,138) 
	rgb255=(252,141,89) 
	rgb255=(227,74,51) 
	rgb255=(179,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd7seq}{
	rgb255=(254,240,217) 
	rgb255=(253,212,158) 
	rgb255=(253,187,132) 
	rgb255=(252,141,89) 
	rgb255=(239,101,72) 
	rgb255=(215,48,31) 
	rgb255=(153,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd9seq}{
	rgb255=(255,247,236) 
	rgb255=(254,232,200) 
	rgb255=(253,212,158) 
	rgb255=(253,187,132) 
	rgb255=(252,141,89) 
	rgb255=(239,101,72) 
	rgb255=(215,48,31) 
	rgb255=(179,0,0) 
	rgb255=(127,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={Paired4qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
}}
\pgfplotsset{/pgfplots/colormap={Paired6qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
}}
\pgfplotsset{/pgfplots/colormap={Paired8qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
	rgb255=(253,191,111) 
	rgb255=(255,127,0) 
}}
\pgfplotsset{/pgfplots/colormap={Paired10qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
	rgb255=(253,191,111) 
	rgb255=(255,127,0) 
	rgb255=(202,178,214) 
	rgb255=(106,61,154) 
}}
\pgfplotsset{/pgfplots/colormap={Paired12qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
	rgb255=(253,191,111) 
	rgb255=(255,127,0) 
	rgb255=(202,178,214) 
	rgb255=(106,61,154) 
	rgb255=(255,255,153) 
	rgb255=(177,89,40) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel14qual}{
	rgb255=(251,180,174) 
	rgb255=(179,205,227) 
	rgb255=(204,235,197) 
	rgb255=(222,203,228) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel16qual}{
	rgb255=(251,180,174) 
	rgb255=(179,205,227) 
	rgb255=(204,235,197) 
	rgb255=(222,203,228) 
	rgb255=(254,217,166) 
	rgb255=(255,255,204) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel18qual}{
	rgb255=(251,180,174) 
	rgb255=(179,205,227) 
	rgb255=(204,235,197) 
	rgb255=(222,203,228) 
	rgb255=(254,217,166) 
	rgb255=(255,255,204) 
	rgb255=(229,216,189) 
	rgb255=(253,218,236) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel23qual}{
	rgb255=(179,226,205) 
	rgb255=(253,205,172) 
	rgb255=(203,213,232) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel25qual}{
	rgb255=(179,226,205) 
	rgb255=(253,205,172) 
	rgb255=(203,213,232) 
	rgb255=(244,202,228) 
	rgb255=(230,245,201) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel27qual}{
	rgb255=(179,226,205) 
	rgb255=(253,205,172) 
	rgb255=(203,213,232) 
	rgb255=(244,202,228) 
	rgb255=(230,245,201) 
	rgb255=(255,242,174) 
	rgb255=(241,226,204) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG3div}{
	rgb255=(233,163,201) 
	rgb255=(247,247,247) 
	rgb255=(161,215,106) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG5div}{
	rgb255=(208,28,139) 
	rgb255=(241,182,218) 
	rgb255=(247,247,247) 
	rgb255=(184,225,134) 
	rgb255=(77,172,38) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG7div}{
	rgb255=(197,27,125) 
	rgb255=(233,163,201) 
	rgb255=(253,224,239) 
	rgb255=(247,247,247) 
	rgb255=(230,245,208) 
	rgb255=(161,215,106) 
	rgb255=(77,146,33) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG9div}{
	rgb255=(197,27,125) 
	rgb255=(222,119,174) 
	rgb255=(241,182,218) 
	rgb255=(253,224,239) 
	rgb255=(247,247,247) 
	rgb255=(230,245,208) 
	rgb255=(184,225,134) 
	rgb255=(127,188,65) 
	rgb255=(77,146,33) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG11div}{
	rgb255=(142,1,82) 
	rgb255=(197,27,125) 
	rgb255=(222,119,174) 
	rgb255=(241,182,218) 
	rgb255=(253,224,239) 
	rgb255=(247,247,247) 
	rgb255=(230,245,208) 
	rgb255=(184,225,134) 
	rgb255=(127,188,65) 
	rgb255=(77,146,33) 
	rgb255=(39,100,25) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn4div}{
	rgb255=(123,50,148) 
	rgb255=(194,165,207) 
	rgb255=(166,219,160) 
	rgb255=(0,136,55) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn6div}{
	rgb255=(118,42,131) 
	rgb255=(175,141,195) 
	rgb255=(231,212,232) 
	rgb255=(217,240,211) 
	rgb255=(127,191,123) 
	rgb255=(27,120,55) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn8div}{
	rgb255=(118,42,131) 
	rgb255=(153,112,171) 
	rgb255=(194,165,207) 
	rgb255=(231,212,232) 
	rgb255=(217,240,211) 
	rgb255=(166,219,160) 
	rgb255=(90,174,97) 
	rgb255=(27,120,55) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn10div}{
	rgb255=(64,0,75) 
	rgb255=(118,42,131) 
	rgb255=(153,112,171) 
	rgb255=(194,165,207) 
	rgb255=(231,212,232) 
	rgb255=(217,240,211) 
	rgb255=(166,219,160) 
	rgb255=(90,174,97) 
	rgb255=(27,120,55) 
	rgb255=(0,68,27) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu3seq}{
	rgb255=(236,231,242) 
	rgb255=(166,189,219) 
	rgb255=(43,140,190) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu5seq}{
	rgb255=(241,238,246) 
	rgb255=(189,201,225) 
	rgb255=(116,169,207) 
	rgb255=(43,140,190) 
	rgb255=(4,90,141) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu7seq}{
	rgb255=(241,238,246) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(116,169,207) 
	rgb255=(54,144,192) 
	rgb255=(5,112,176) 
	rgb255=(3,78,123) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu9seq}{
	rgb255=(255,247,251) 
	rgb255=(236,231,242) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(116,169,207) 
	rgb255=(54,144,192) 
	rgb255=(5,112,176) 
	rgb255=(4,90,141) 
	rgb255=(2,56,88) 
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn4seq}{
	rgb255=(246,239,247) 
	rgb255=(189,201,225) 
	rgb255=(103,169,207) 
	rgb255=(2,129,138) 
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn6seq}{
	rgb255=(246,239,247) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(103,169,207) 
	rgb255=(28,144,153) 
	rgb255=(1,108,89) 
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn8seq}{
	rgb255=(255,247,251) 
	rgb255=(236,226,240) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(103,169,207) 
	rgb255=(54,144,192) 
	rgb255=(2,129,138) 
	rgb255=(1,100,80) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr3div}{
	rgb255=(241,163,64) 
	rgb255=(247,247,247) 
	rgb255=(153,142,195) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr5div}{
	rgb255=(230,97,1) 
	rgb255=(253,184,99) 
	rgb255=(247,247,247) 
	rgb255=(178,171,210) 
	rgb255=(94,60,153) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr7div}{
	rgb255=(179,88,6) 
	rgb255=(241,163,64) 
	rgb255=(254,224,182) 
	rgb255=(247,247,247) 
	rgb255=(216,218,235) 
	rgb255=(153,142,195) 
	rgb255=(84,39,136) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr9div}{
	rgb255=(179,88,6) 
	rgb255=(224,130,20) 
	rgb255=(253,184,99) 
	rgb255=(254,224,182) 
	rgb255=(247,247,247) 
	rgb255=(216,218,235) 
	rgb255=(178,171,210) 
	rgb255=(128,115,172) 
	rgb255=(84,39,136) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr11div}{
	rgb255=(127,59,8) 
	rgb255=(179,88,6) 
	rgb255=(224,130,20) 
	rgb255=(253,184,99) 
	rgb255=(254,224,182) 
	rgb255=(247,247,247) 
	rgb255=(216,218,235) 
	rgb255=(178,171,210) 
	rgb255=(128,115,172) 
	rgb255=(84,39,136) 
	rgb255=(45,0,75) 
}}
\pgfplotsset{/pgfplots/colormap={PuRd4seq}{
	rgb255=(241,238,246) 
	rgb255=(215,181,216) 
	rgb255=(223,101,176) 
	rgb255=(206,18,86) 
}}
\pgfplotsset{/pgfplots/colormap={PuRd6seq}{
	rgb255=(241,238,246) 
	rgb255=(212,185,218) 
	rgb255=(201,148,199) 
	rgb255=(223,101,176) 
	rgb255=(221,28,119) 
	rgb255=(152,0,67) 
}}
\pgfplotsset{/pgfplots/colormap={PuRd8seq}{
	rgb255=(247,244,249) 
	rgb255=(231,225,239) 
	rgb255=(212,185,218) 
	rgb255=(201,148,199) 
	rgb255=(223,101,176) 
	rgb255=(231,41,138) 
	rgb255=(206,18,86) 
	rgb255=(145,0,63) 
}}
\pgfplotsset{/pgfplots/colormap={Purples3seq}{
	rgb255=(239,237,245) 
	rgb255=(188,189,220) 
	rgb255=(117,107,177) 
}}
\pgfplotsset{/pgfplots/colormap={Purples5seq}{
	rgb255=(242,240,247) 
	rgb255=(203,201,226) 
	rgb255=(158,154,200) 
	rgb255=(117,107,177) 
	rgb255=(84,39,143) 
}}
\pgfplotsset{/pgfplots/colormap={Purples7seq}{
	rgb255=(242,240,247) 
	rgb255=(218,218,235) 
	rgb255=(188,189,220) 
	rgb255=(158,154,200) 
	rgb255=(128,125,186) 
	rgb255=(106,81,163) 
	rgb255=(74,20,134) 
}}
\pgfplotsset{/pgfplots/colormap={Purples9seq}{
	rgb255=(252,251,253) 
	rgb255=(239,237,245) 
	rgb255=(218,218,235) 
	rgb255=(188,189,220) 
	rgb255=(158,154,200) 
	rgb255=(128,125,186) 
	rgb255=(106,81,163) 
	rgb255=(84,39,143) 
	rgb255=(63,0,125) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu4div}{
	rgb255=(202,0,32) 
	rgb255=(244,165,130) 
	rgb255=(146,197,222) 
	rgb255=(5,113,176) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu6div}{
	rgb255=(178,24,43) 
	rgb255=(239,138,98) 
	rgb255=(253,219,199) 
	rgb255=(209,229,240) 
	rgb255=(103,169,207) 
	rgb255=(33,102,172) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu8div}{
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(209,229,240) 
	rgb255=(146,197,222) 
	rgb255=(67,147,195) 
	rgb255=(33,102,172) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu10div}{
	rgb255=(103,0,31) 
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(209,229,240) 
	rgb255=(146,197,222) 
	rgb255=(67,147,195) 
	rgb255=(33,102,172) 
	rgb255=(5,48,97) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy3div}{
	rgb255=(239,138,98) 
	rgb255=(255,255,255) 
	rgb255=(153,153,153) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy5div}{
	rgb255=(202,0,32) 
	rgb255=(244,165,130) 
	rgb255=(255,255,255) 
	rgb255=(186,186,186) 
	rgb255=(64,64,64) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy7div}{
	rgb255=(178,24,43) 
	rgb255=(239,138,98) 
	rgb255=(253,219,199) 
	rgb255=(255,255,255) 
	rgb255=(224,224,224) 
	rgb255=(153,153,153) 
	rgb255=(77,77,77) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy9div}{
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(255,255,255) 
	rgb255=(224,224,224) 
	rgb255=(186,186,186) 
	rgb255=(135,135,135) 
	rgb255=(77,77,77) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy11div}{
	rgb255=(103,0,31) 
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(255,255,255) 
	rgb255=(224,224,224) 
	rgb255=(186,186,186) 
	rgb255=(135,135,135) 
	rgb255=(77,77,77) 
	rgb255=(26,26,26) 
}}
\pgfplotsset{/pgfplots/colormap={RdPu4seq}{
	rgb255=(254,235,226) 
	rgb255=(251,180,185) 
	rgb255=(247,104,161) 
	rgb255=(174,1,126) 
}}
\pgfplotsset{/pgfplots/colormap={RdPu6seq}{
	rgb255=(254,235,226) 
	rgb255=(252,197,192) 
	rgb255=(250,159,181) 
	rgb255=(247,104,161) 
	rgb255=(197,27,138) 
	rgb255=(122,1,119) 
}}
\pgfplotsset{/pgfplots/colormap={RdPu8seq}{
	rgb255=(255,247,243) 
	rgb255=(253,224,221) 
	rgb255=(252,197,192) 
	rgb255=(250,159,181) 
	rgb255=(247,104,161) 
	rgb255=(221,52,151) 
	rgb255=(174,1,126) 
	rgb255=(122,1,119) 
}}
%EDIT: Added number of classes
\pgfplotsset{/pgfplots/colormap={RedsSeq}{
	rgb255=(254,229,217)
	rgb255=(252,174,145)
	rgb255=(251,106,74)
	rgb255=(222,45,38)
	rgb255=(165,15,21)
}}

\pgfplotsset{/pgfplots/colormap={Reds3seq}{
	rgb255=(254,224,210) 
	rgb255=(252,146,114) 
	rgb255=(222,45,38) 
}}
\pgfplotsset{/pgfplots/colormap={Reds5seq}{
	rgb255=(254,229,217) 
	rgb255=(252,174,145) 
	rgb255=(251,106,74) 
	rgb255=(222,45,38) 
	rgb255=(165,15,21) 
}}
\pgfplotsset{/pgfplots/colormap={Reds7seq}{
	rgb255=(254,229,217) 
	rgb255=(252,187,161) 
	rgb255=(252,146,114) 
	rgb255=(251,106,74) 
	rgb255=(239,59,44) 
	rgb255=(203,24,29) 
	rgb255=(153,0,13) 
}}
\pgfplotsset{/pgfplots/colormap={Reds9seq}{
	rgb255=(255,245,240) 
	rgb255=(254,224,210) 
	rgb255=(252,187,161) 
	rgb255=(252,146,114) 
	rgb255=(251,106,74) 
	rgb255=(239,59,44) 
	rgb255=(203,24,29) 
	rgb255=(165,15,21) 
	rgb255=(103,0,13) 
}}

\pgfplotsset{/pgfplots/colormap={RdYlBuSeq}{
	rgb255=(165,0,38) 
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(171,217,233) 
	rgb255=(116,173,209) 
	rgb255=(69,117,180) 
	rgb255=(49,54,149) 
}}

\pgfplotsset{/pgfplots/colormap={RdYlBu4div}{
	rgb255=(215,25,28) 
	rgb255=(253,174,97) 
	rgb255=(171,217,233) 
	rgb255=(44,123,182) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu6div}{
	rgb255=(215,48,39) 
	rgb255=(252,141,89) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(145,191,219) 
	rgb255=(69,117,180) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu8div}{
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(171,217,233) 
	rgb255=(116,173,209) 
	rgb255=(69,117,180) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu10div}{
	rgb255=(165,0,38) 
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(171,217,233) 
	rgb255=(116,173,209) 
	rgb255=(69,117,180) 
	rgb255=(49,54,149) 
}}
%END EDIT

\pgfplotsset{/pgfplots/colormap={RdYlGn3div}{
	rgb255=(252,141,89) 
	rgb255=(255,255,191) 
	rgb255=(145,207,96) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn5div}{
	rgb255=(215,25,28) 
	rgb255=(253,174,97) 
	rgb255=(255,255,191) 
	rgb255=(166,217,106) 
	rgb255=(26,150,65) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn7div}{
	rgb255=(215,48,39) 
	rgb255=(252,141,89) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(217,239,139) 
	rgb255=(145,207,96) 
	rgb255=(26,152,80) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn9div}{
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(217,239,139) 
	rgb255=(166,217,106) 
	rgb255=(102,189,99) 
	rgb255=(26,152,80) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn11div}{
	rgb255=(165,0,38) 
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(217,239,139) 
	rgb255=(166,217,106) 
	rgb255=(102,189,99) 
	rgb255=(26,152,80) 
	rgb255=(0,104,55) 
}}
\pgfplotsset{/pgfplots/colormap={Set14qual}{
	rgb255=(228,26,28) 
	rgb255=(55,126,184) 
	rgb255=(77,175,74) 
	rgb255=(152,78,163) 
}}
\pgfplotsset{/pgfplots/colormap={Set16qual}{
	rgb255=(228,26,28) 
	rgb255=(55,126,184) 
	rgb255=(77,175,74) 
	rgb255=(152,78,163) 
	rgb255=(255,127,0) 
	rgb255=(255,255,51) 
}}
\pgfplotsset{/pgfplots/colormap={Set18qual}{
	rgb255=(228,26,28) 
	rgb255=(55,126,184) 
	rgb255=(77,175,74) 
	rgb255=(152,78,163) 
	rgb255=(255,127,0) 
	rgb255=(255,255,51) 
	rgb255=(166,86,40) 
	rgb255=(247,129,191) 
}}
\pgfplotsset{/pgfplots/colormap={Set23qual}{
	rgb255=(102,194,165) 
	rgb255=(252,141,98) 
	rgb255=(141,160,203) 
}}
\pgfplotsset{/pgfplots/colormap={Set25qual}{
	rgb255=(102,194,165) 
	rgb255=(252,141,98) 
	rgb255=(141,160,203) 
	rgb255=(231,138,195) 
	rgb255=(166,216,84) 
}}
\pgfplotsset{/pgfplots/colormap={Set27qual}{
	rgb255=(102,194,165) 
	rgb255=(252,141,98) 
	rgb255=(141,160,203) 
	rgb255=(231,138,195) 
	rgb255=(166,216,84) 
	rgb255=(255,217,47) 
	rgb255=(229,196,148) 
}}
\pgfplotsset{/pgfplots/colormap={Set33qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
}}
\pgfplotsset{/pgfplots/colormap={Set35qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
}}
\pgfplotsset{/pgfplots/colormap={Set37qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
	rgb255=(253,180,98) 
	rgb255=(179,222,105) 
}}
\pgfplotsset{/pgfplots/colormap={Set39qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
	rgb255=(253,180,98) 
	rgb255=(179,222,105) 
	rgb255=(252,205,229) 
	rgb255=(217,217,217) 
}}
\pgfplotsset{/pgfplots/colormap={Set311qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
	rgb255=(253,180,98) 
	rgb255=(179,222,105) 
	rgb255=(252,205,229) 
	rgb255=(217,217,217) 
	rgb255=(188,128,189) 
	rgb255=(204,235,197) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral3div}{
	rgb255=(252,141,89) 
	rgb255=(255,255,191) 
	rgb255=(153,213,148) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral5div}{
	rgb255=(215,25,28) 
	rgb255=(253,174,97) 
	rgb255=(255,255,191) 
	rgb255=(171,221,164) 
	rgb255=(43,131,186) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral7div}{
	rgb255=(213,62,79) 
	rgb255=(252,141,89) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(230,245,152) 
	rgb255=(153,213,148) 
	rgb255=(50,136,189) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral9div}{
	rgb255=(213,62,79) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(230,245,152) 
	rgb255=(171,221,164) 
	rgb255=(102,194,165) 
	rgb255=(50,136,189) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral11div}{
	rgb255=(158,1,66) 
	rgb255=(213,62,79) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(230,245,152) 
	rgb255=(171,221,164) 
	rgb255=(102,194,165) 
	rgb255=(50,136,189) 
	rgb255=(94,79,162) 
}}
\pgfplotsset{/pgfplots/colormap={YlGn4seq}{
	rgb255=(255,255,204) 
	rgb255=(194,230,153) 
	rgb255=(120,198,121) 
	rgb255=(35,132,67) 
}}
\pgfplotsset{/pgfplots/colormap={YlGn6seq}{
	rgb255=(255,255,204) 
	rgb255=(217,240,163) 
	rgb255=(173,221,142) 
	rgb255=(120,198,121) 
	rgb255=(49,163,84) 
	rgb255=(0,104,55) 
}}
\pgfplotsset{/pgfplots/colormap={YlGn8seq}{
	rgb255=(255,255,229) 
	rgb255=(247,252,185) 
	rgb255=(217,240,163) 
	rgb255=(173,221,142) 
	rgb255=(120,198,121) 
	rgb255=(65,171,93) 
	rgb255=(35,132,67) 
	rgb255=(0,90,50) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu3seq}{
	rgb255=(237,248,177) 
	rgb255=(127,205,187) 
	rgb255=(44,127,184) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu5seq}{
	rgb255=(255,255,204) 
	rgb255=(161,218,180) 
	rgb255=(65,182,196) 
	rgb255=(44,127,184) 
	rgb255=(37,52,148) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu7seq}{
	rgb255=(255,255,204) 
	rgb255=(199,233,180) 
	rgb255=(127,205,187) 
	rgb255=(65,182,196) 
	rgb255=(29,145,192) 
	rgb255=(34,94,168) 
	rgb255=(12,44,132) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu9seq}{
	rgb255=(255,255,217) 
	rgb255=(237,248,177) 
	rgb255=(199,233,180) 
	rgb255=(127,205,187) 
	rgb255=(65,182,196) 
	rgb255=(29,145,192) 
	rgb255=(34,94,168) 
	rgb255=(37,52,148) 
	rgb255=(8,29,88) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr4seq}{
	rgb255=(255,255,212) 
	rgb255=(254,217,142) 
	rgb255=(254,153,41) 
	rgb255=(204,76,2) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr6seq}{
	rgb255=(255,255,212) 
	rgb255=(254,227,145) 
	rgb255=(254,196,79) 
	rgb255=(254,153,41) 
	rgb255=(217,95,14) 
	rgb255=(153,52,4) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr8seq}{
	rgb255=(255,255,229) 
	rgb255=(255,247,188) 
	rgb255=(254,227,145) 
	rgb255=(254,196,79) 
	rgb255=(254,153,41) 
	rgb255=(236,112,20) 
	rgb255=(204,76,2) 
	rgb255=(140,45,4) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd3seq}{
	rgb255=(255,237,160) 
	rgb255=(254,178,76) 
	rgb255=(240,59,32) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd5seq}{
	rgb255=(255,255,178) 
	rgb255=(254,204,92) 
	rgb255=(253,141,60) 
	rgb255=(240,59,32) 
	rgb255=(189,0,38) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd7seq}{
	rgb255=(255,255,178) 
	rgb255=(254,217,118) 
	rgb255=(254,178,76) 
	rgb255=(253,141,60) 
	rgb255=(252,78,42) 
	rgb255=(227,26,28) 
	rgb255=(177,0,38) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd9seq}{
	rgb255=(255,255,204) 
	rgb255=(255,237,160) 
	rgb255=(254,217,118) 
	rgb255=(254,178,76) 
	rgb255=(253,141,60) 
	rgb255=(252,78,42) 
	rgb255=(227,26,28) 
	rgb255=(189,0,38) 
	rgb255=(128,0,38) 
}}

